EarthNet2021: A novel large-scale dataset and challenge for forecasting localized climate impacts

Climate change is global, yet its concrete impacts can strongly vary between different locations in the same region. Seasonal weather forecasts currently operate at the mesoscale (> 1 km). For more targeted mitigation and adaptation, modelling impacts to < 100 m is needed. Yet, the relationship between driving variables and Earth's surface at such local scales remains unresolved by current physical models. Large Earth observation datasets now enable us to create machine learning models capable of translating coarse weather information into high-resolution Earth surface forecasts. Here, we define high-resolution Earth surface forecasting as video prediction of satellite imagery conditional on mesoscale weather forecasts. Video prediction has been tackled with deep learning models. Developing such models requires analysis-ready datasets. We introduce EarthNet2021, a new, curated dataset containing target spatio-temporal Sentinel 2 satellite imagery at 20 m resolution, matched with high-resolution topography and mesoscale (1.28 km) weather variables. With over 32000 samples it is suitable for training deep neural networks. Comparing multiple Earth surface forecasts is not trivial. Hence, we define the EarthNetScore, a novel ranking criterion for models forecasting Earth surface reflectance. For model intercomparison we frame EarthNet2021 as a challenge with four tracks based on different test sets. These allow evaluation of model validity and robustness as well as model applicability to extreme events and the complete annual vegetation cycle. In addition to forecasting directly observable weather impacts through satellite-derived vegetation indices, capable Earth surface models will enable downstream applications such as crop yield prediction, forest health assessments, coastline management, or biodiversity monitoring. Find data, code, and how to participate at www.earthnet.tech .

==> sections/OLD02relatedwork.tex <==
\section{Related work}

\paragraph{Traditional approaches to the forecasting of Earth surface}
Our work relates to both spatial downscaling of climate or coarse-scale remote sensing data and to temporal forecasts. Temporal forecasts of vegetation state have been performed on km to 50 km scale \citet{tadesse2010,asoka2015,kraft2019}.  Approaches to downscale Earth surface conditions to <100m exist as well, but are not connected to temporal forecasts to our knowledge, but rather blending multiple observations \citet{ke2016}. 

\paragraph{ML approaches to the forecasting of Earth surface}
Using temporal context (\citet{kraft2019} and \citet{foley2020}) using spatial context (Chris). Both useful at improving performance, but no dataset available allow to use both spatial and temporal context -> Ideal for video prediction models.


==> sections/ideas2022.tex <==
EarthNet2022
    Go Worldwide
    Go to 10m/pix from 20m?pix
    Go 256x256
    Go with more sentinel bands
    Go with other source for weather (global)
    Add GLiM predictor (soil/geology)
    Add QQ
    Improve metrics based on learnings from 2021
    DL based cloud mask
